A Feasibility Study of a Soft, Low-Cost, 6-Axis Load Cell for Haptics

Haptic devices have shown to be valuable in supplementing surgical training, especially when providing haptic feedback based on user performance metrics such as wrench applied by the user on the tool. However, current 6-axis force/torque sensors are prohibitively expensive. This paper presents the design and calibration of a low-cost, six-axis force/torque sensor specially designed for laparoscopic haptic training applications. The proposed design uses Hall-effect sensors to measure the change in the position of magnets embedded in a silicone layer that results from an applied wrench to the device. Preliminary experimental validation demonstrates that these sensors can achieve an accuracy of 0.45 N and 0.014 Nm, and a theoretical XY range of +/-50N, Z range of +/-20N, and torque range of +/-0.2Nm. This study indicates that the proposed low-cost 6-axis force/torque sensor can accurately measure user force and provide useful feedback during laparoscopic training on a haptic device.

==> nomenclature.tex <==
\section{Modeling Nomenclature}
%%%%%%%%%% NOMENCLATURE TABLE %%%%%%%%%%
\bgroup
\def\arraystretch{1.5}%
\begin{table}[h]
	\centering
	\footnotesize
	\caption{Nomenclature}
	\begin{tabular}{m{0.07\columnwidth} m{.8\columnwidth}}
		\hline
		\textbf{Symbol} & \textbf{Description} \\
		\hline
		\{F\}
		& A right-handed coordinate frame.\\
		\hdashline
        \{0\} &  The frame located at the center of the sensor \\
		\hdashline
        $\Rot{a}{b}$ & A rotation matrix describing the orientation of frame $\{B\}$ relative to frame $\{A\}$.\\
        \hdashline
          $\mb{x}^\wedge$ & 
          The . 
           \begin{equation*}
                 \mb{x}^\wedge=\begin{cases}
			         \begin{bmatrix} 
                        0 & -x_3 & x_2 \\
                        x_3 & 0 & -x_1\\
                        -x_2 & x_1 & 0
                        \end{bmatrix} \in so(3) & \textrm{for~} \mb{x}=\begin{bmatrix}
                            x_1 \\ x_2 \\x_3
                        \end{bmatrix}\\
                      \begin{bmatrix}
                        \bs{\omega}^\wedge & \mb{v} \\ 
                        \mb{0} & 0
                      \end{bmatrix} \in se(3)  &
                      \mb{x}=\begin{bmatrix}\mb{v}\in\realfield{3} \\ \bs{\omega}\in\realfield{3} \end{bmatrix}              
		      \end{cases}
            \end{equation*}    
        \\	
    \hdashline
    $\left(\mb{X}\right)^\vee$ & 
    An inverse operator of $(\cdot)^\wedge$ such that:
    \begin{equation*}
        \mb{X}^\vee=\begin{cases}
			[x_1, x_2, x_3]\T, & \textrm{for~} \mb{X}\in so(3)\\
                [\mb{v}\T, \bs{\omega}\T]\T, & \textrm{for~} \mb{X}^\wedge = \begin{bmatrix}\bs{\omega}^\wedge & \mb{v} \\ \mb{0} & 0\end{bmatrix} \in se(3)
		 \end{cases}
   \end{equation*}    
    \\
    \hdashline
    $\log\left(\mb{T}\right)$ & 
    The matrix logarithm $\log(\cdot):~SE(3)\rightarrow se(3)$.
    \begin{equation*}
       \log\left(\mb{T}\right) = \begin{bmatrix}\bs{\omega}^\wedge & \mb{v} \\ \mb{0} & 0\end{bmatrix}\in se(3) 
   \text{ for }\mb{T}\in SE(3)\end{equation*}    
    \\
    \hdashline
    $\mb{I}_n$ & An $n\times n$ identity matrix\\\hline
    \end{tabular}
    \label{tab:nomenclature}
\end{table}
\egroup
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
